What Makes Effective Leadership in Agile Software Development Teams?

Effective leadership is one of the key drivers of business and project success, and one of the most active areas of management research. But how does leadership work in agile software development, which emphasizes self-management and self-organization and marginalizes traditional leadership roles? To find out, this study examines agile leadership from the perspective of thirteen professionals who identify as agile leaders, in different roles, at ten different software development companies of varying sizes. Data from semi-structured interviews reveals that leadership: (1) is dynamically shared among team members; (2) engenders a sense of belonging to the team; and (3) involves balancing competing organizational cultures (e.g. balancing the new agile culture with the old milestone-driven culture). In other words, agile leadership is a property of a team, not a role, and effectiveness depends on agile team members' identifying with the team, accepting responsibility, and being sensitive to cultural conflict.

==> tables/analysistables.tex <==
\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Analysis table for Dynamic Team Leadership -- Team members that drive the work forward}
\label{tab:result1}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Dynamic Team Leadership  &``team members share responsibility'' & Have team members that take initiative and responsibility & ``Another guy said, `well you won't have the time, so I'm the Scrum Master now.' And that was it. That was the decision, and it was very natural, so they don't see the scrum master as a person, they see it as a role that they all can take. Take the weight off someone else's shoulders and help out.'' & I1\\
\hline
Dynamic Team Leadership  &``team members don't drive work'' & Have team members that take initiative and responsibility & ``To be totally honest we also in the beginning made staffing decisions based on that. Where we said: `This is just not working out', with someone who is just passive, and does not create this active work-mode. Then of course, they were not happy and they said, `oh, we don't want to be on that project,' and then we happily let them go. And then tried to rearrange.'' & G3\\
\hline
Dynamic Team Leadership  &``manager dependence'' & Have team members that take initiative and responsibility & ``It's not depending on if we use waterfall projects or agile, projects do have problems, and when they do, we need to have some sort of leadership in the teams in order to solve some of those problems. That is for us the main challenge; how we get somebody to come from an outside world where the personal always had a manger that she or he can refer to, and when things get stressful there is always someone to tap them on the back and say `OK, everything's gonna be fine!' While we try to have a company where everyone's responsible for their own mistakes and they are responsible for their own work. That's hard! Really hard!'' & J1\\
\hline
Dynamic Team Leadership  &``no shared responsibility'' & Have team members that take initiative and responsibility & ``And the ability to basically design things; form and shape things, which also brings me to think of that agile work is probably not for everyone. You need to have people who basically are willing to take responsibility, who are willing to get empowered and to make decisions.'' & B1\\
\hline
Dynamic Team Leadership  &``focus on collaboration'' & Have team members that take initiative and responsibility & ``My own anecdotal perspective is that for the teams that are doing it right, and by right I mean that they are embracing the principles and not just delivering things in a short amount of time. They are really thinking about being collaborative and self-organized and all those things. They become passionate about it and really want to do more of it.'' & C1\\
\hline
Dynamic Team Leadership  &``motivated teammembers'' & Have team members that take initiative and responsibility & ``I took the project over and it was about 3 weeks behind and we made up all that time. I liken that progress to having used this Scrum framework, because it was just… God! Everybody got awake and in line and moving, and communicating.'' & G1\\
\hline

\end{tabular}
\end{table*}



\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Analysis table for Dynamic Team Leadership -- Let team members lead}
\label{tab:result2}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Dynamic Team Leadership  &``listen to team input'' & Let team members lead & ``Not only regarding stories and requirements, but if they have other ideas of improving teams or whatever, if we talk to them and try to fix it, they really like it. Their input is important. This is the main factor to happiness at work here, as I see it.'' & H1\\
\hline
Dynamic Team Leadership  &``initiate team-drive'' & Let team members lead & ``For example, the need to learn TDD so we get together and I teach them and then I feel like, if I stay around they'll be dependent on me much longer. So I have to step back and disappear for like two weeks and then I get back to the project. I'm more of a consultant in that team than a developer.'' & I1\\
\hline
Dynamic Team Leadership  &``team members lead'' & Let team members lead & ``I guess we were just really lucky with the team members we had. This was basically also my objective; careful! Don't become a project manager, don't start planning stuff, don't start assigning or defining tasks. Stay out of that!'' & G3\\
\hline
Dynamic Team Leadership  &``afraid to share leadership'' & Let team members lead & ``So maybe we're killing the leadership instinct in them by exposing them to strong leadership from the beginning.'' & I1\\
\hline
Dynamic Team Leadership  &``team members lead'' & Let team members lead & ``The formality there might be the problem. Or it is formal because... well I've asked them, and the reason it's formal is that the two leaders don't feel like they can leave it to the other people. So they don't trust the other team members and there is a person there that could be a leader and sometimes the person tries and he dies... like the person's leadership is not enough. The person's leadership is not enough to overpower the other ones, so sometimes I sit with the person and say `so, I know you see that problem, because I see your face and you are seeing that problem, so what are you going to do about it?' Then the person gets motivated and tries again and then he... I also say to the other ones to be quiet and just listen. My hope is that it helps in the long term, that that person that has strong opinions and actually fighting for it, will motivate the other people in the team to do the same. And that the two leaders that don't usually listen to the rest of the team will learn that they should listen more.'' & I1\\
\hline
Dynamic Team Leadership  &``leadership not shared'' & Let team members lead & ``There are teams that have a strong leadership, and there the problem is another one which is this whole idea of having someone telling everybody what to do. For me, it's the leadership will make it the best or the worst.'' & J1\\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Analysis table for Dynamic Team Leadership -- Step in, if needed}
\label{tab:result3}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Dynamic Team Leadership  &``leaders intervene'' & Step in, if needed & ``I could [force the teams to try a practice]. And I did, actually, a couple of times and the way I do this is, I have a plan and then I plan a presentation or a small workshop with the team to show them the problems they have right now. Then I say, well let's try this other process, and I explain it to them and they will try it for 2 weeks. And if they don't like it, they're free to go back to the old one.'' & I1\\
\hline
Dynamic Team Leadership  &``leaders intervene'' & Step in, if needed & ``Most of the time we have to interfere as leaders in order to help the team come together and make a better decision, in relation to how to attend a client request. But that makes this whole thing much harder because I need to have independent developers and testers and designers that are able to talk to clients most of the time.'' & J1\\
\hline
Dynamic Team Leadership  &``leaders intervene'' & Step in, if needed & ``What's mostly happening is that they come to me and say `what I think I'm seeing is this, do you agree with that?' They have the sense of that I'm always watching what's going on.'' & I1\\
\hline
\end{tabular}
\end{table*}





\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Social identity -- Build a strong social identity across functions}
\label{tab:result4}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Social identity  &``include more people'' & Build a strong social identity across functions & ``A new resource from finance for example didn't use to have much to do with the other functions. Now with these meetings and planning, they are all one team working together and cheer each other's aspects. So new members quickly become a part of that family, which is a really interesting byproduct.'' & F1\\
\hline
Social identity  &``broaden their perspective and create a common identity'' & Build a strong social identity across functions & ``It's very easy to see that, well `my part in the project is just coding,' but that's not quite true. They get less cohesive by having a clear separation of roles.'' & H1\\
\hline

\end{tabular}
\end{table*}



\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Social identity -- Create an IT and business\slash customer partnership}
\label{tab:result5}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Social identity  &``dev.\ and business'' & Create an IT and business\slash customer partnership & ``The teams are fairly self-organizing, and the team is composed of business and IT sitting together for dedicated work sessions. So it's a dedicated team.'' & A1\\
\hline
Social identity  &``engagement with the business-side'' & Create an IT and business\slash customer partnership & ``The business partnership and engagement you create is absolutely tremendous compared to the traditional approach! /\ldots/ I can feel that the people simply like what they're doing. Yes. Absolutely. And the reason why there is increased job satisfaction is, well first of all it's working as one team, it's not us and them; IT versus Business.'' & B1\\
\hline
Social identity  &``create a common identity with customers'' & Create an IT and business\slash customer partnership & ``We say ``you are responsible with us for the success of this project.'' So we try to have the client as the product owner. Usually, the one that's responsible for the project, well, that would be a dream come true if all project had the client as the product owner, but that's not always possible.'' & J1\\
\hline
Social identity  &``not business versus us'' & Create an IT and business\slash customer partnership & ``So they can again, work to be a part of and share the accountability [in agile]. I mean, for a whole variety of reasons that involvement of the business partner as a part of the team, not them versus us, and IT is no longer the scapegoat if they didn't get what they wanted, or we delivered on time or we ran out of money etc.'' & D1\\
\hline
Social identity  & ``business not included'' & Create an IT and business\slash customer partnership & ``Our customer is not easy to get to our meetings. So when we have it, it's too late. And when we have it, most of the times we get change requests and something to change.'' & G2\\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Social identity -- Build a strong team identity}
\label{tab:result6}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Social identity  &``social ceremony'' & Build a strong team identity & ``My team works pretty well, but the clients are next door, literally. The team can walk and talk to them. Very easy. And even talking to [another city] is only an online chat away. It's interesting because when we deploy software in the middle of the day, the [people] here actually call the other units and say "ok, we're stopping the software for a couple of minutes to deploying. So then everyone stops. We could do a night deploy, but we prefer to do that. Our PO finds out stuff from other units when we're doing that so.... the PO is from the commercial/business area and is the person who's been here the second longest. My team is very easy with that. '' & H1\\
\hline
Social identity  &``team ceremonies to build identity'' & Build a strong team identity & ``The Scrum part takes between 7-10 minutes. Then it takes another 5-10 minutes to fill out the time, and it's in the spreadsheet, so then I got to the tab that shows the burn down. People wait for that! Like: `Oooh let's see what the burn-down is today!' And then the third part is just an open forum, an open meeting, and people sort of take care of things that will only take a short amount of time to discuss. If things come up that will take more time then they go ahead and set up their own meetings. So that's how I extend it to accommodate the distance.'' & G1\\
\hline

\end{tabular}
\end{table*}

%\begin{table*}
%\footnotesize
%\renewcommand{\arraystretch}{1.3}
%\caption{Social identity -- Be a prototypical leader}
%\label{tab:result}
%\begin{tabular}{llp{23mm}p{50mm}r}
%\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
%\hline
%Social identity  &``the geek identity'' & Be a prototypical leader & ``We are all geeks in here, and even I, and if necessary I'd be coding to deliver projects, so we tend to focus more on that.'' & I1\\
%Social identity  &``working leader role'' & Be a prototypical leader & ``well sometimes the Scrum Master role is, well, it might be a doer also in some of the cases.'' & G1\\


%\hline
%\end{tabular}
%\end{table*}






\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Organizational Cultures -- tailored approach}
\label{tab:result7}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Organizational Cultures  &``shield to surrounding'' & Tailored approach & ``I don't know if \emph{shield} is the right word, but the team doesn't have to worry. I have a very high-level schedule with milestones that I can show them like `this is where we are.' I have a kind of waterfall-like representation of our sprints and the main milestones and I show that to them. But then I just take care of all the requirements from the organization, you know, at a higher level. The team doesn't have to worry about that stuff. But if they want to see something I have this nice little schedule I can show them. That's where I become a traditional project manager. I would say I spend quite a bit of my time in that role, making sure everything fits the rest of the organization.'' & G1\\
\hline
Organizational Cultures  & ``context of solution'' & Tailored approach & ``What one individual pilot project starts to practice, you always have difficulty scaling that, because that's what they were doing and got really good at doing exactly that specific to that project. But that's not necessarily well translated into practice format across the enterprise. That needs to be more of the fundamentals and the process behind it.'' & A1\\
\hline
Organizational Cultures  & ``make waterfall more incremental'' & Tailored approach & ``So one of the things is that either you break a project into smaller pieces to get it done within 6 months and deliver less capability, but the highest priority capabilities. And that's both for agile and waterfall projects, that the concept is to deliver capability to the business within 6 months, so that the business sees the benefits earlier rather than later. So that is stolen from the agile concept, to deliver incrementally.'' & E2\\
\hline
Organizational Cultures  & ``when agile doesn't fit'' & Tailored approach & ``For example, for the project when we deliver our support package and we are in a test phase, like regression tests. For this period I think agile is not the methodology to use. We have 2 months of which we have our sprint backlog empty, or with just some tasks on quality. We work on internal message we get from our testers. And I think that for that period I don't think we have to use agile methodology.'' & G2\\
\hline
Organizational Cultures  & ``multiple POs'' & Tailored approach & ``Sometimes we run into situations where a team has multiple product owners and that's very difficult to work with, because then you have to balance your priorities across multiple product owners for your team to deliver. So what we try to do is break our teams into small enough groups that we basically have a single product owner for that capability.'' & E2\\
\hline

\end{tabular}
\end{table*}


\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Organizational Cultures -- Understand the company ecosystem}
\label{tab:result8}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Organizational Cultures  &``not just the team itself and its value creation'' & Understand the company ecosystem & ``Also, what adds complexity is what I call the company ecosystem. So the other areas that you need to work on, like if you need a new environment for example, maybe new infrastructure for the teams. If you haven't brought those people along in your agile journey, then subsequently you will have that hurdle to overcome because of the different culture and behaviors.'' & D1\\
\hline
Organizational Cultures  & ``tweak agile'' & Understand the company ecosystem & ``We decided to have a business council instead of a single product owner. On that council I think we are up to 7 people. One from each department. For example, there is one representative for finance, one from marketing, one from operations, etc. These people act as our product owners and we have a 3-week sprint cycle, we meet with them every three weeks and review projects that are currently in process and our first step is to make sure they are still our priorities and we look at the list of priorities that haven't started yet. /.../ I can't tell you how many compliments we've received from the overall business teams at many different levels. Even though it's work for them to sit down and argue back and forth on what is important from a company perspective, we've knocked down all those silos and force them to cooperate and agree that IT is working on the most important projects for the company.'' & F1\\
\hline
Organizational Cultures  & ``silo adaption'' & Understand the company ecosystem & ``To some people it's a subtle difference and they sometimes have a hard time grasping why we don't just have one list for finance, one list for sales ops etc. But it has been a key drive for us since we have shared resources, to have one cross-functional list.'' & F1\\
\hline
Organizational Cultures  & ``old-type projects'' & Understand the company ecosystem & ``I've been working with companies that want to `install' agile, like it's not a cultural change, they think it's a software like Microsoft Office or something. One thing that actually helps a lot is that even when you're deciding which project to take on, that project has to have a few principles that will improve the whole group or organization. So if you're working in a company, or on a project that has been sold as a fixed price and fixed scope project, you won't be able to really have profound conversations on how to improve as a group, and you're just running to meet deadlines on scope.'' & J1\\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Organizational Cultures -- Adapt to customer culture}
\label{tab:result9}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Organizational Cultures  & ``customer culture'' & Adapt to customer culture & ``Sometime it's just not responsible or feasible to try to get things into production every two weeks, let's say. I mean, that's just wouldn't make sense. So, how we try to circumvent that, or even from our customers' perspective (our business partners), often they don't want changes as often as we could deliver them.'' & C1\\
\hline
Organizational Cultures  & ``customer transparency'' & Adapt to customer culture & ``The sprint review has been a Godsend because we pull in the stakeholders, and again, they understand much earlier in the process how things are going, what we discovered, and we can set their expectations of what the final packages actually are going to be. They can see it, and they can see it working. So I would say that and the other thing is: I think it does (maybe this sound like a contradiction) but it does nurture discipline, because of this regular rhythm.'' & G1\\%Lucas: does this one fit?
\hline
Organizational Cultures  & ``adapt to project characteristics'' & Adapt to customer culture & ``We try to set the restrictions so that people know when they are NOT following them. We use to work mostly with start-up companies, and with start-up companies, that's a big discussion because with a tight budget, why could you have 17 layers of tests? when you instead could have really compact objective test that test throughout the whole business process. So why build this big infrastructure of testing when you don't know if the company will even exist a month from now? So that's why we have restrictions and not rules. If they decide on that particular project that they don't have to have a big focus on testing, they do have to have some tests, that's what the restrictions say to them, but they can discuss it and decide what's best for them.'' & J1\\
\hline
Organizational Cultures  & ``change in contracting'' & Adapt to customer culture & ``Most of our contracts are based on agile principles. Their scope is not defined, or usually, they're quite loosely defined. We often have team contracts, which is when we set up a team that team is fully focused on that project. We don't have one person on multiple teams, as you can see in a normal software house. We have full-time dedicated developers for each project.'' & J1\\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1.3}
\caption{Organizational Cultures -- Adjust ``old'' behavior}
\label{tab:result10}
\begin{tabular}{llp{23mm}p{50mm}r}
\bfseries Theme & \bfseries Initial category name & \bfseries Final Category name & \bfseries Example Quote & \bfseries PID\\
\hline
Organizational Cultures  & ``old behavior'' & Adjust ``old'' behavior & ``We've trained them over the years that they only have one shot at it. So they strive to get everything in and described, thinking I only have one shot at this, because usually we run out of money or run out of time.'' & D1\\
\hline
Organizational Cultures  & ``difficulty of change'' & Adjust ``old'' behavior & ``What I understood very early was that waterfall approach provides some very familiar and comfortable handrails, called milestones, which everybody grasps and clings to for life. This takes this away, so in the beginning people are... the stress level does go up with people who are not familiar with this, because they fell that there's no certainty: `where are we going? What are we doing? How come we only focus on the next three weeks?' That the hardest thing I think for people.'' & G1\\
\hline
Organizational Cultures  & ``old habits'' & Adjust ``old'' behavior & ``I mean typical misunderstandings like to what they were used to, they were giving money to IT and of course they wanted to know what they would get at the end of the year for their money. We told them: `sorry, we can't tell you.' `Why can't you tell us?' `Because we are agile and our backlog changes continuously, so we can't tell you what you get in the end of the year, but we can tell you that if we all do our jobs right, then at the end of the year whatever you have will be exactly what the end-users need, or at least from their top priority.' Sure that was new, it was a bit hard to swallow. But then it was accepted and the business organization is now really behind it.'' & G3\\
\hline
Organizational Cultures  & ``behavioral change'' & Adjust ``old'' behavior & ``The biggest challenge for me is the behavioral one. Everyone has to behave differently and with everyone I mean developers, product owners, scrum masters, but also of course business stakeholders, line managers, and I really mean everyone. /.../ Allowing the team to become a high performance team without the problem of having a lot of politics involved in the execution of the project.'' & E2\\
\hline
Organizational Cultures  & ``change in project follow-up'' & Adjust ``old'' behavior & ``We made clear that we don't work against people's heads or slides, we work against the backlog and the backlog is prioritized by the product owner based on end-user feedback. And it really worked, so from then on, in these days we have very very good support for the whole thing.'' & G3\\
\hline


\end{tabular}
\end{table*}





